Machine learning for subgroup discovery under treatment effect

In many practical tasks it is needed to estimate an effect of treatment on individual level. For example, in medicine it is essential to determine the patients that would benefit from a certain medicament. In marketing, knowing the persons that are likely to buy a new product would reduce the amount of spam. In this chapter, we review the methods to estimate an individual treatment effect from a randomized trial, i.e., an experiment when a part of individuals receives a new treatment, while the others do not. Finally, it is shown that new efficient methods are needed in this domain.

==> makefile <==
MAIN_FILE = my_chapter
MAIN_FILE_COMPILE=$(MAIN_FILE).tex
PRECOMPIELD_NAME=precompiled
PRECOMPIELD_DEP=$(shell ./find-deps.bash "template_settings/ch_static_preamble.tex")
TIKZFLD = ./tikz/

RMFILESLIST = *.mtc* *.aux *.bak *.bbl *.bcf *.blg *.log *.out *.toc *.tdo _region.* *.run.xml *.flg *.idx *.maf _region_.* *~ *.ilg *.ind  *.fls *.fdb_latexmk *.M* *.gz *.fmt \#* *.nav *.snm precompiled.pdf
RMFILESCMD = $(patsubst %,-iname "%" -o,$(RMFILESLIST)) -false

TIME     = /usr/bin/time -p
LATEXMK  = latexmk -halt-on-error -pdf -pdflatex="pdflatex --shell-escape -fmt $(PRECOMPIELD_NAME) --synctex=1 -interaction=nonstopmode" # -shell-escape" 
FMTPDFLATEX=pdftex -ini -jobname="$(PRECOMPIELD_NAME)" -interaction=nonstopmode "&pdflatex" mylatexformat.ltx 

PDFLATEX = pdflatex -interaction=nonstopmode -output-directory 
PDFCROP  = pdfcrop
RM       = /bin/rm -f

StandAloneGraphicsTeXFiles = $(wildcard $(TIKZFLD)/*.tex)

PDFGraphics = $(patsubst %.tex,%.pdf,$(StandAloneGraphicsTeXFiles))

#LatexFiles = $(shell find . -path $(TIKZFLD) -prune -o -type f -iname '*.tex')
LatexFiles = $(shell ./find-deps.bash "$(MAIN_FILE).tex")

CurrentInclude = $(shell ./find-include.bash "$(MAIN_FILE).tex" "" $(CurrentFile))
CurrentIncludeGUARDSuffix = \#INCLUDE\#
CurrentIncludeGUARD = $(patsubst %,%$(CurrentIncludeGUARDSuffix),$(CurrentInclude))

#Includes = $(shell ./extract-includes.bash '\input{$(MAIN_FILE)}')
#IncludesPDF = $(patsubst %.tex,%.pdf,$(Includes))
#IncludesAUX = $(patsubst %.tex,%.aux,$(Includes))

COMPILE = $(TIME) $(LATEXMK) -jobname=$(MAIN_FILE) $(MAIN_FILE_COMPILE)
COMPILE_ALL = $(COMPILE) 

#----------------------init done--------------------------------

default : $(MAIN_FILE).pdf

# No difference for fast and standard in the case of small documents
#fast : $(CurrentIncludeGUARD)
fast : $(MAIN_FILE).pdf

# Forcing to recompile every time, latexmk will make a check
.PHONY : FORCE_MAKE
$(MAIN_FILE).pdf : $(MAIN_FILE).bcf $(PRECOMPIELD_NAME).fmt $(MAIN_FILE).tex $(LatexFiles) $(PDFGraphics) my_folder/my_biblio.bib FORCE_MAKE
	$(COMPILE_ALL)

$(MAIN_FILE).bcf : FORCE_MAKE
	test ! -f $(MAIN_FILE).bcf || grep '</bcf:controlfile>' $(MAIN_FILE).bcf || ( echo 'BCF file is corrupted, removing...' && rm $(MAIN_FILE).bcf )

$(PRECOMPIELD_NAME).fmt : $(PRECOMPIELD_DEP)
	touch $(PRECOMPIELD_NAME).mtc0
	$(FMTPDFLATEX)  $(MAIN_FILE_COMPILE)

$(TIKZFLD)%.pdf : $(TIKZFLD)%.tex
	$(PDFLATEX) $(TIKZFLD) $< 

my_folder/my_biblio.bib : /home/leshyk/PhD/library.bib
	/home/leshyk/PhD/Gits/Scripts/correct-library-mendeley.bash
	/home/leshyk/PhD/Gits/Scripts/clear-library.sh
	cp /home/leshyk/PhD/library.bib my_folder/my_biblio.bib

clean : .PHONY
	@find $(RMFILESCMD) | xargs -I{} rm -r '{}'

depclean : clean
	$(RM) $(TIKZFLD)*.pdf
	#$(RM) $(IncludesPDF)

distclean : depclean
	$(RM) $(MAIN_FILE).pdf

noop : .PHONY
	@echo 'noop DONE'
#------------------------------------------------------
# for fast compiling of one include
.SECONDEXPANSION:

$(CurrentIncludeGUARD) : %$(CurrentIncludeGUARDSuffix) : $$(shell ./find-deps.bash %.tex) $(PRECOMPIELD_NAME).fmt $(MAIN_FILE).tex $(PDFGraphics) FORCE_MAKE
	@sed -i 's+\\begin{document}+\\includeonly{$(patsubst %$(CurrentIncludeGUARDSuffix),%,$@)}\\begin{document}+' $(MAIN_FILE_COMPILE)
	$(COMPILE) && echo "Compiled" >> $@

#--------------------------------------------------------
# For fast compiling of chapters. Syncinc will not work.

#incr: $(IncludesPDF) 
	#pdftk $(IncludesPDF) cat output $(MAIN_FILE).pdf

#.SECONDEXPANSION:

#$(IncludesPDF): %.pdf: %.tex $$(shell ./find-deps.bash %.tex) $(MAIN_FILE).tex $(PRECOMPIELD_NAME).fmt  $(PDFGraphics) 
## Checking if all aux exists. If not should recompile all.
#$(CHECK_AUX_COMPILE_ALL)
#cp $(MAIN_FILE).tex $(MAIN_FILE_COMPILE)
#sed -i 's+\\begin{document}+\\includeonly{$(patsubst %.pdf,%,$@)}\\begin{document}+' $(MAIN_FILE_COMPILE)
#$(TIME) $(LATEXMK) '-jobname=$(MAIN_FILE)' $(MAIN_FILE_COMPILE)
#cp $(MAIN_FILE).pdf $@



==> my_folder/tex/definition-example.tex <==
\begin{m-definition}[хороший и-тест] %при необходимости в [] можно записать название определения или убрать его
	\label{def:ex}
	% \index только для принятых работ
	% шаблон записи определения в Предметный указатель 
	\index[ru]{название\_определения!1-3 уточняющих слова или~ничего}
	\index[en]{definition\_title!1-3 words for detail or~without "!-part}
	% пример записи определения в Предметный указатель 
	\index[ru]{и-тест!хороший!наилучший}
	\index[en]{i-test!good!best}
	% пример записи определения в Предметный указатель 
	\index[ru]{и-тест!замкнутый}
	\index[en]{i-test!closed}
	В тексте определения только {\itshape важные термины} выделяются курсивом. Если определение носит лишь вспомогательный характер, то допустимо не использовать окружение \texttt{m-definition}, представляя текст определения в обычном абзаце. Ключевые термины при этом обязательно выделяются курсивом.
\end{m-definition}

==> my_folder/tex/pseudocode-agl-DTestsFDScaling.tex <==
	\begin{algorithm} %[h]
		\SetKwFunction{algoDTestsFDSCALING}{} 
		\SetKwProg{myalg}{Algorithm}{}{} %write in 2nd agrument <<Algorithm>>, <<Procedure>> etc
		\nonl\myalg{\algoDTestsFDSCALING}{
			\KwInput{the many-valued context $\cont[M]\eqdef(G,M,W,J)$, the class membership $\epsilon: G\to K$} 
			\KwOutput{positive and negative binary contexts $\overbar{\cont[K]_+}\eqdef(\overbar{G_+},M,I_+)$, $\overbar{\cont[K]_-}\eqdef(\overbar{G_-},M,I_-)$ such that i-tests found in $\overbar{\cont[K]_+}$ are diagnostic tests in $\cont[M]$, and objects from $\overbar{\cont[K]_-}$ are counter-examples} %последние строки формируют начальное множество диагностических тестов
			\For {$\forall g_i,$ $g_j \in G$\label{step:FD-scaling-first-step}}{
				%(\tcp*[f]{possible inlined comment})
				\If{$i < j$ }{
					$\overbar{G} \leftarrow (g_i,g_j)$\;
				}
			}
			%		$M\leftarrow M\setminus k$\;
			\For {$\forall (g_i,g_j)\in \overbar{G}$}{
				%(\tcp*[f]{possible inlined comment})
				\If{$m(g_i) = m(g_j)$ }{ %на самом деле здесь цикл по всем компонентам вектора-строки
					$(g_i,g_j) I m$\; % or setI() function
				}
				\uIf{$\epsilon(g_i) = \epsilon(g_j)$ }{
					$\overbar{G_+} \leftarrow (g_i,g_j)$\;
				}
				\lElse{$\overbar{G_-} \leftarrow (g_i,g_j)$\label{FD-scaling-step-last}}	
			}		
			$I_+= I\cap (\overbar{G_+}\times M)$, $I_-= I\cap (\overbar{G_-}\times M)$\label{FD-scaling-step-newK}\; 
			\For {$\forall \overbar{g_+}\in \overbar{G_+}$, $\forall \overbar{g_-}\in \overbar{G_-}$ }{
				\If{$\overbar{g_+}\uA \subseteq \overbar{g_-}\uA$ }{
					$\overbar{G_+} \leftarrow \overbar{G_+} \setminus \overbar{g_+}$\;
				}
			}
			%		\Return \;
		}
		\caption{Псевдокод алгоритма \texttt{DiagnosticTestsScalingAndInferring} \cite{Naidenova2017}}\label{alg:AlgoFDSCALING}
		% example of adding an item to Index
		% \index for accepted papers only
		\index[ru]{алгоритм!\texttt{название\_алгоритма}} 
		% key words <<алгоритм>> и <<algorithm>> keep unmodified
		\index[en]{algorithm!\texttt{algorighm\_title}}
		% authors can used the key word <<процедура>> (procedure) и т.п.
		%
		%
	    % another example:
		\index[ru]{алгоритм!\texttt{DiagnosticTestsScaling\-AndInferring}} %нужен ручной перенос \- из-за ошибки в MakeIndex для команды \texttt
		%ключевые слова <<алгоритм>> и <<algorithm>> не менять
		\index[en]{algorithm!\texttt{DiagnosticTestsScaling\-AndInferring}} %нужен ручной перенос \- из-за ошибки в MakeIndex для команды \texttt
	\end{algorithm} 
	
	% another example of adding an arbitrary keyword to Index
	% some useful keywords: theorem, proposition, lemma, equation etc
	% please, use short keywords (2-3 max)
	\index[ru]{длинное-название-возможное-например-на-немецком} % длинные названия первого уровня как правило запрещены
	\index[en]{long-title-possible-for-example-in-German} 
	
Обратим внимание, что можно сослаться на строчку \ref{step:FD-scaling-first-step} псевдокода из рисунка \ref{alg:AlgoFDSCALING}. 

==> my_folder/tex/rules-list-of-environments.tex <==
Для удобства авторов некоторые названия стандартных окружений приведены в таблице \ref{tab:enum-std}. В таблице \ref{tab:enum-spbpu}  перечислены имена специально разработанных окружений для пакетов SPbPU.

% и примеры их оформления на псевдокоде (см. \cite{cite-spbpu-bci}).


%https://tex.stackexchange.com/questions/2651/should-i-use-center-or-centering-for-figures-and-tables


	\begin{table} [htbp]% Пример записи таблицы с номером, но без отображаемого наименования
	\centering
	\caption{Описание некоторых стандартных \LaTeX{} окружений, рекомендуемых к использования в шаблонах SPbPU}%
	\label{tab:enum-std}
		\begin{SingleSpace}
		%		\resizebox{1\linewidth| &!| &
		\begin{tabular}{|l|p{11cm}|} 
			\hline
			Название окружения&Назначение\\
			\hline
			\verb|center| & центрирование, аналог команды \verb|\centering|, но с добавлением нежелательного пробела, поэтому лучше избегать применения \verb|center|; \\
			\verb|itemize| &{перечисления, в которых нет необходимости нумеровать  пункты, см. подробнее подраздел \ref{sec:strct-and-enum};}\\
			\verb|enumerate| & перечисления с нумерацией, см. подробнее подраздел \ref{sec:strct-and-enum}; \\
			\verb|refsection| & создание отдельных библиографических списков для глав; \\
			\verb|tabular| & оформление таблиц; \\
			\verb|table|   &{автоматическое перемещение по тексту таблиц, оформленных, например, с помощью \verb|tabular|, для минимизации пустых пространств;} \\
			\verb|longtable| & оформление многостраничных таблиц; \\
			\verb|tikzpicture| & создание иллюстраций с помощью пакета \verb|tikz| \cite{ctan-tikz}; \\
			\verb|figure| &{автоматическое перемещение по тексту рисунков, оформленных например, с помощью \verb|tikz| или подключенных с помощью команды \verb|\includegraphics|, для минимизации пустых пространств;}\\
			\verb|subfigure| & оформление вложенных рисунков в составе \verb|figure|; \\
			\verb|algorithm| &{оформление псевдокода на основе пакета \verb|algorithm2e| \cite{ctan-algorithm2e};} \\
			\verb|minipage| & {оформление рисунков и таблиц без функций автоматического перемещения по тексту для  минимизации пустых пространств;} \\
			\verb|equation| & {оформление выключенных (не встроенных в текст с помощью \verb|$...$|) одиночных формул на одной строке;} \\
			\verb|multilined| &{оформление выключенных (не встроенных в текст с помощью \verb|$...$|) одиночных формул в несколько строк;} \\ 
			\verb|aligned| &{оформление нескольких формул с выравниванием по символу \verb|&|.} \\
			\hline		
		\end{tabular}	
		%		}
	\end{SingleSpace}
	\end{table}

На базе пакета \verb|tikz| разработано большое количество расширений \cite{ctan-tikz}, например, \verb|tikzcd|, которые мы рекомендуем использовать для оформления иллюстраций.

	\begin{table} [htbp]% Пример записи таблицы с номером, но без отображаемого наименования
	\centering
	\caption{Описание специально разработанных \LaTeX{} окружений, рекомендуемых к использования в шаблонах SPbPU}%
	\label{tab:enum-spbpu}
	\begin{SingleSpace}
		%		\resizebox{1\linewidth| &!| &
		\begin{tabular}{|l|l|}
			\hline
			Название окружения & Текстово-графический объект\\
			\hline
			\verb|abstr|	 & реферат (abstract); \\
			\verb|m-theorem| & теорема; \\ 
			\verb|m-corollary| & следствие; \\
			\verb|m-proposition| & утверждение; \\
			\verb|m-lemma|   & лемма; \\
			\verb|m-axiom| & аксиома; \\
			\verb|m-example| & пример; \\
			\verb|m-definition| &  определение; \\
			\verb|m-condition| & условие;\\
			\verb|m-problem| & проблема; \\
			\verb|m-exercise| & упраженение;\\
			\verb|m-question| & вопрос;\\
			\verb|m-hypothesis| & гипотеза;\\
			\verb|m-task| & задание. \\
			\hline		
		\end{tabular}	
		%		}
	\end{SingleSpace}
\end{table}

В случае, если авторам потребовалось новое окружение, то создать его можно в файле в файле \texttt{my\_fol\-der/{}my\_set\-tings.tex} согласно правилам, приведённым ниже.

\begin{enumerate}[1.]
	\item Для перехода в режим создания окружений следует указать:
	\begin{itemize}
		\item \verb|\theoremstyle{myplain}| --- окружения с доказательствами или аксиомами;
		\item \verb|\theoremstyle{mydefinition}| --- окружения, не связанные с доказательствами или аксиомами.
	\end{itemize}
	\item В команде создания окружения следует ввести краткий псевдоним (\verb|m-new-env|) и отображаемое в pdf имя окружения (\verb|Название_окружения|):
	\begin{itemize}
		\item \texttt{\textbackslash{}newtheorem\{m-new-env-second\}\{Название\_окруже\-ния\}\-[chap\-ter]}.
	\end{itemize}
\end{enumerate}


%\begin{m-new-env-first}
%	Тест первого пользовательского окружения
%\end{m-new-env-first}
%
%\begin{m-new-env-second}
%	Тест второго пользовательского окружения
%\end{m-new-env-second}

==> my_folder/tex/rules-theorem-like-expressions.tex <==
Вопросы форматирования текстово-графических объектов (окружений) не регламентированы в известных нам ГОСТах, поэтому предлагаем придерживаться следующих правил:

\begin{itemize}
	\item \textbf{полужирный текст} рекомендуем использовать только для названий стандартных окружений с нумерационной частью, например, \textbf{определение 1.1}, \textbf{теорема 2.2}, \textbf{пример 2.3}, \textbf{лемма 4.5};
	
	\item \textit{курсив} рекомендуем использовать только для выделения переменных в формулах, служебной информации об авторах главы (статьи), важных терминов, представляемых по тексту, а также для всего тела окружений, связанных с получением \textit{новых существенных результатов и их доказательством}: теорема, лемма, следствие, утверждение и другие.
\end{itemize}



==> my_folder/tex/theorem-example.tex <==
\begin{m-theorem}[о неполноте] %при необходимости в [] можно записать название теоремы или убрать его
	\label{th:ex} 
	% \index только для принятых работ
	% шаблон записи теоремы в Предметный указатель
	\index[ru]{теорема!название\_теоремы или о чём} %ключевое слово <<теорема>> не менять
	\index[en]{theorem!1-3 words for detail or description}
	% пример записи алгоритма в Предметный указатель
	\index[ru]{теорема!о неполноте}
	\index[en]{theorem!about incompleteness}
	% пример записи алгоритма в Предметный указатель
	\index[ru]{теорема!о жизни}
	\index[en]{theorem!about life}
	Текст теоремы полностью выделен курсивом. Допустимо математические символы не выделять курсивом, если это искажает их значения. Используется абзацный отсуп, так как ``Абзацы в тексте начинают отступом'' в соответствии с ГОСТ 2.105--95. Название теоремы допустимо убрать.
\end{m-theorem}
Доказательство теоремы \ref{th:ex}, леммы, утверждений, следствий и других завершаем символом белого квадрата (номер символа в Юникод 25A1) без выравнивания по правому краю. $\square$

Тело доказательства не выделяется курсивом.
Тело следующих окружений также не выделяется сплошным курсивом: определение, условие, проблема, пример, упражнение, вопрос, гипотеза и другие.

==> template_settings/ch_dynamic_preamble.tex <==
%%% Предметный указатель  ГОСТ 7.78-99 Index %%%
%c обобщенными рубриками или развернутый
%или указатель терминов (в общем случае - произвольное число указателей)
%подключать до hyperref

%\usepackage{makeidx} %возможно, необходимо подключить И/ИЛИ пройти Tools-> Commands -> MakeIndex

\usepackage{imakeidx} 
%\indexsetup{level=\section*,toclevel=section,noclearpage}
\makeindex[program=makeindex,
options=-s template_settings/common/myindex.ist, %подключаем стилевой файл для форматирования вывода
name=ru, % префикс для русских указателей 
% если убрать <<ru>>, то для работы дефолтового придется вручную включать Tools-> Commands -> MakeIndex
title={\chapterLight{} 
%   \hrule{}
	Предметный указатель
%	\hrule{}
} 
%,columns=1 %по умолчанию 2
]
\makeindex[program=makeindex,
options=-s template_settings/common/myindex.ist, %подключаем стилевой файл для форматирования вывода
name=en, % префикс для английских указателей
title={\chapterLight{}
%	\hrule{}
	Index
%	\hrule{}
} 
%,columns=1 %по умолчанию 2
] 
%убрать добавление <<title>> в содержание:
%\noindexintoc %not to add index title in PURE makeidx %intoc is false by default with imakeidx

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% FROM DISERTATION %%%%%%%%%%%%%%%%%%%%%
%%% Алгоритмы %%%

%\usepackage[linesnumbered]{algorithm2e}
\usepackage[linesnumbered,vlined,figure,scleft]{algorithm2e}

%% Glogal params %%
%ruled, tworuled, algoruled --- put lines to wrap the caption plus a line at the bottom (top) - one should not use this together with inline captions!
%vlined 										--- instead of begin...end will be lines
%boxed 											--- make a box
% figure 										--- count as Fig. ...


% Settings of caption       --- if one will use \caption{} option 	instead of inline + environment caption.
%\SetAlgoCaptionSeparator{.}
%\SetAlgorithmName{Algorithm}{} %last arg is the title of listing table


% Settings for lines numbers
\SetNlSkip{0em}							% sets the value of the space between the line numbers and the text, by default 1em.
\SetNlSty{normalsize}{\hphantom{0}}{.}%defines how to print line numbers
%\hspace*{5mm} does not work 
\SetAlgoNlRelativeSize{-1}	% sets the relative size of line numbers. By default, line numbers are two size smaller than algorithm text

% How to ignore line nuber and to wrap
%http://tex.stackexchange.com/questions/153646/algorithm2e-disabling-line-numbers-for-specific-lines
%http://tex.stackexchange.com/questions/86580/how-to-adjust-line-numbers-of-algorithm2e-package
\makeatletter
%\newcommand{\nosemic}{\renewcommand{\@endalgocfline}{\relax}}% Drop semi-colon ;
%\newcommand{\dosemic}{\renewcommand{\@endalgocfline}{\algocf@endline}}% Reinstate semi-colon ;
%\newcommand{\pushline}{\Indp}% Indent
%\newcommand{\popline}{\Indm\dosemic}% Undent
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\makeatother


% Settings for vlines 			
%\SetInd{0.3em}{0.5em}			%default and spaces before and after are 0.5em and 1em
%\SetVlineSkip{5em}					% Sets the value of the vertical space after the little horizontal line which closes a block in vlined mode

%% User abbreviations for ASTRA %%
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
%% See also %%
%http://tex.stackexchange.com/questions/145114/caption-below-boxed-algorithm2e-when-used-as-a-figure
%http://tex.stackexchange.com/questions/83536/align-comments-in-algorithm-with-package-algorithm2e



==> template_settings/ch_static_preamble.tex <==
\input{template_settings/ch_preamble} % please, keep unmodified


==> template_settings/index.tex <==
{\smallA %
	\printindex[ru]% печатаем
} %end of \smallA
\newpage % 

==> template_settings/indexEng.tex <==
{\smallA %
	\pdfbookmark[-1]{Index}{ind}
\addtocruNoProtect{chapter}{Предметный указатель} % Add to TOC in Russian
\addtocenNoProtect{chapter}{Index} % Add to TOC in Russian
	\printindex[en]% печатаем
%	}
} %end of \smallA
\newpage % 
